Complex Hadamard Matrices - Quantum Symmetries, Equivalence and Non-Local Games

We consider quantum group generalizations of the action of monomial matrices on complex Hadamard matrices. This gives rise to various notions of quantum symmetries and quantum equivalences of Hadamard matrices. We show that if one acts by a certain largest monomial quantum group, then all Hadamard matrices of a given size become quantum equivalent. Taking a more restrictive quantization leads to a notion of $s$-quantum equivalence. We exhibit examples of Butson matrices of the same size and order that are not $s$-quantum equivalent for any choice of $s$. We also show that $s$-quantum equivalence is operationally modeled by a synchronous non-local ``Hadamard equivalence'' game. Our methods are largely graphical calculus based, using categories generated by complementary spiders. We use these same tools to study quantum affine equivalence of quantum groups, and prove that all finite quantum groups of the same size are quantum affinely equivalent. We also provide a short graphical proof of a result of Kasprzak--So\l tan--Woronowicz asserting that quantum symmetries of finite quantum groups must be classical.

==> strdiag.tex <==
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric} 
\usetikzlibrary{shapes.symbols} 
\def\Dcup{\Diagram{\draw (1,1) .. controls +(down:0.5) and +(down:0.5) .. (2,1);}}
\def\Dcap{\Diagram{\draw (1,0) .. controls +(up:0.5) and +(up:0.5) .. (2,0);}}
\def\Did{\Diagram{\draw (1,0) -- (1,1);}}
\def\Dcross{\Diagram{\draw (0,0) -- (1,1);\draw (1,0) -- (0,1);}}

\def\Rcup{\Diagram{\draw[mid arrow] (1,1) .. controls +(down:0.5) and +(down:0.5) .. (2,1);}}
\def\Lcup{\Diagram{\draw[mid arrow] (2,1) .. controls +(down:0.5) and +(down:0.5) .. (1,1);}}
\def\Rcap{\Diagram{\draw[mid arrow] (1,0) .. controls +(up:0.5) and +(up:0.5) .. (2,0);}}
\def\Lcap{\Diagram{\draw[mid arrow] (2,0) .. controls +(up:0.5) and +(up:0.5) .. (1,0);}}
\def\Fid{\Diagram{\draw[mid arrow] (1,0) -- (1,1);}}
\def\Bid{\Diagram{\draw[mid arrow] (1,1) -- (1,0);}}
\def\Fcross{\Diagram{\draw[->] (0,0) -- (1,1);\draw[->] (1,0) -- (0,1);}}

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}

\def\Diagram#1{%
\thinspace\textchoice
{\DiagramA{0.25em}{1em}{1em}{#1}}
{\DiagramA{0.25em}{0.7em}{1em}{#1}}
{\DiagramA{0.175em}{0.55em}{0.7em}{#1}}
{\DiagramA{0.125em}{0.4em}{0.5em}{#1}}
{\DiagramA{0.25em}{0.7em}{1em}{#1}}%
\thinspace%
}

\def\DiagramA#1#2#3#4{%
%\expandafter\tikzpicture\Gparam
\tikzpicture[
	%arrow styles
	mid arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .5 with {\arrow{>}}
      }}},
	late arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .8 with {\arrow{>}}
      }}},
	%point styles
	circ/.style={circle,draw,fill=white,inner sep=1pt},
	bcirc/.style={circle,draw,fill=black,inner sep=1pt},
	map/.style={draw,fill=white,trapezium,trapezium left angle=90,trapezium right angle=120,inner sep=1pt},
	mapC/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=90,inner sep=1pt},
	mapT/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=90,inner sep=1pt},
	mapA/.style={draw,fill=white,trapezium,trapezium left angle=90,trapezium right angle=60,inner sep=1pt},
	selfC/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=120,inner sep=1pt},
	selfCR/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=60,inner sep=1pt},
	selfT/.style={draw,fill=white,trapezium,trapezium left angle=60,trapezium right angle=120,inner sep=1pt},
	selfTR/.style={draw,fill=white,trapezium,trapezium left angle=120,trapezium right angle=60,inner sep=1pt},
	selfA/.style={draw,fill=white,signal,signal to=east,inner sep=1pt},
	selfAR/.style={draw,fill=white,signal,signal to=west,inner sep=1pt},
	square/.style={draw,fill=white,rectangle,inner sep=1pt},
	vec/.style={draw,fill=white,isosceles triangle, shape border rotate=-90,isosceles triangle apex angle=60,inner sep=1pt},
	covec/.style={draw,fill=white,isosceles triangle, shape border rotate=90,isosceles triangle apex angle=60,inner sep=1pt},
]
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Dlinewidth em}
#4
\endtikzpicture
}

\def\Dlinewidth{0.05}

\def\DstringsB #1/#2(#3,#4){
\ifnum#1>0
\pgfmathparse{#3-(#1-1)/2}
\let\x=\pgfmathresult
\pgfmathparse{#3+(#1-1)/2}
\let\xx=\pgfmathresult
\foreach \a in {\x,...,\xx}
	\draw (\a,#4-\Dyshift) .. controls +(up:0.25) .. (#3,#4);
\fi
\ifnum#2>0
\pgfmathparse{#3-(#2-1)/2}
\let\x=\pgfmathresult
\pgfmathparse{#3+(#2-1)/2}
\let\xx=\pgfmathresult
\foreach \a in {\x,...,\xx}
	\draw (\a,#4+\Dyshift) .. controls +(down:0.25) .. (#3,#4);
\fi
}

\newcount\tmpcount
\def\Dcount#1{\ifx/#1/\else\advance\tmpcount by1\fihere\Dcount\fi}

\def\DstringsC [#1/#2](#3,#4){
\tmpcount=-1
\Dcount#1//
\pgfmathparse{#3-\the\tmpcount/2}
\let\x=\pgfmathresult
\scope[
	up arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .3 with {\arrow{>}}
      }}},
	down arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .3 with {\arrow{<}}
      }}},
]
\DstringsD{#3}{#4}#1//
\endscope
\tmpcount=-1
\Dcount#2//
\pgfmathparse{#3-\the\tmpcount/2}
\let\x=\pgfmathresult
\scope[
	down arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .7 with {\arrow{>}}
      }}},
	up arrow/.style={postaction={decorate,decoration={
        markings,
        mark=at position .7 with {\arrow{<}}
      }}},
]
\DstringsE{#3}{#4}#2//
\endscope
}

\def\fihere#1\fi{\fi#1}
\def\DstringsD#1#2#3{\ifx/#3/\else
	\csname D#3\endcsname (\x,#2-\Dyshift) .. controls +(up:0.25) .. (#1,#2);
	\pgfmathparse{\x+1}
	\let\x=\pgfmathresult
	\fihere\DstringsD{#1}{#2}\fi
}
\def\DstringsE#1#2#3{\ifx/#3/\else
	\csname D#3\endcsname (\x,#2+\Dyshift) .. controls +(down:0.25) .. (#1,#2);
	\pgfmathparse{\x+1}
	\let\x=\pgfmathresult
	\fihere\DstringsE{#1}{#2}\fi
}

\def\Dstrings{
\futurelet\nextchar\DstringsA
}

\def\DstringsA{\ifx[\nextchar\let\next=\DstringsC\else\let\next=\DstringsB\fi\next}

\def\Dmor#1#2 (#3,#4){
\def\Dyshift{0.5}
\ifx;#2;\else\Dstrings#2(#3,#4)\fi
\node at (#3,#4) [#1] {};
}

\def\DMor#1#2 (#3,#4)#5{
\def\Dyshift{1}
\ifx;#2;\else\Dstrings#2(#3,#4)\fi
\node at (#3,#4) [#1] {#5};
}

\def\spider{\futurelet\nextchar\spiderA}
\def\spiderA{\ifx[\nextchar\def\next[##1]{\Diagram{\Dmor{bcirc}[##1] (1,0.5)}}\else\def\next##1{\Diagram{\Dmor{bcirc}##1 (1,0.5)}}\fi\next}
\def\wspider{\futurelet\nextchar\wspiderA}
\def\wspiderA{\ifx[\nextchar\def\next[##1]{\Diagram{\Dmor{circ}[##1] (1,0.5)}}\else\def\next##1{\Diagram{\Dmor{circ}##1 (1,0.5)}}\fi\next}

\def\Ddef#1#2{\expandafter\def\csname D#1\endcsname{#2}}
\Ddef>{\draw[<-]}
\Ddef<{\draw[>-]}
\Ddef-{\draw}
\expandafter\def\csname D0\endcsname#1;{}
\expandafter\def\csname D.\endcsname (#1,#2)#3;{\node at (#1,#2) {$\dots$};}

\endinput

